Large-Scale Zero-Shot Image Classification from Rich and Diverse Textual Descriptions

We study the impact of using rich and diverse textual descriptions of classes for zero-shot learning (ZSL) on ImageNet. We create a new dataset ImageNet-Wiki that matches each ImageNet class to its corresponding Wikipedia article. We show that merely employing these Wikipedia articles as class descriptions yields much higher ZSL performance than prior works. Even a simple model using this type of auxiliary data outperforms state-of-the-art models that rely on standard features of word embedding encodings of class names. These results highlight the usefulness and importance of textual descriptions for ZSL, as well as the relative importance of auxiliary data type compared to algorithmic progress. Our experimental results also show that standard zero-shot learning approaches generalize poorly across categories of classes.

==> tables/exclude_groups.tex <==
\begin{table*}[h]\centering
\caption{\textbf{Effect of excluding a category of classes from
    the training set on ZSL performance.} Results on the mp500 test
  split when the ZSL model is trained with a category of classes
  removed. Specifically we compare excluding all \textit{animal} classes Vs. excluding the
  same number of random \textit{non-animal} classes. We repeat the same process
  for the \textit{plant} class. The ZSL model we use is our top performing
  CADA-VAE model trained on the Wikipedia articles using
  ALBERT-xxlarge features. The performance numbers quoted, on the relevant
  class categories, are from one training run of the model. The
  numbers in row 1 and row 3 clearly show the performance on the unseen animal classes drops
  dramatically when the animal classes are removed from the training set.
}
\ra{1.3}
{
\begin{tabular}{@{}*{1}{l}*{7}{r}@{}}
  \toprule
  ALBERT-xxlarge & & \multicolumn{6}{c}{\textbf{Performance on class categories in mp500 (\%)}}\\
  \cmidrule(l){3-8}
  & & \multicolumn{2}{c}{\textbf{animals} (82)} &
  \multicolumn{2}{c}{\textbf{plants} (39)} &
  \multicolumn{2}{c}{\textbf{remain.} (368)}\\
  \cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8}
  \textbf{Classes excluded} & \textbf{\# excluded} & top-1
  & top-5     & top-1     & top-5      & top-1
  & top-5 \\
  \midrule
  None & 0 & 23.84           & 58.92          & 3.43           & 13.82
  & 19.78          & 45.23 \\
  All animal & 398  & 1.94            & 8.13           & 3.69  & 13.65
  & 20.67          & 45.51 \\
  Random non-animal & 398 & 22.54   & 59.87          & 2.67           & 11.65          & 11.52          & 32.69 \\
  All plant & 31                   & 24.84           & 60.12          & 1.07           & 5.68           & 19.88          & 45.30              \\
  Random non-plant & 31               & 24.53           & 58.14          & 3.05           & 11.82          & 19.88          & 45.39\\
\bottomrule
\end{tabular}
}
\label{tbl:exclude_groups}


\begin{tabular}{@{}*{1}{l}*{7}{r}@{}}
  \toprule
  GloVe & & \multicolumn{6}{c}{\textbf{Performance on class categories in mp500 (\%)}}\\
  \cmidrule(l){3-8}
  & & \multicolumn{2}{c}{\textbf{animals} (82)} &
  \multicolumn{2}{c}{\textbf{plants} (39)} &
  \multicolumn{2}{c}{\textbf{remain.} (368)}\\
  \cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8}
  \textbf{Classes excluded} & \textbf{\# excluded} & top-1
  & top-5     & top-1     & top-5      & top-1
  & top-5 \\
  \midrule
  None              & 0     & 30.41 & 65.32     &  5.32 & 19.57     & 22.90 & 51.98     \\
  All animal        & 398   &  3.52 & 16.56     &  4.47 & 17.70     & 23.36 & 52.98     \\
  Random non-animal & 398   & 28.74 & 60.60     &  5.59 & 21.62     & 15.32 & 41.72     \\
  All plant         & 31    & 29.56 & 63.08     &  3.92 & 16.18     & 22.64 & 52.32     \\
  Random non-plant  & 31    & 28.29 & 62.29     &  6.00 & 21.26     & 22.61 & 52.34     \\
\bottomrule
\end{tabular}


\begin{tabular}{@{}*{1}{l}*{7}{r}@{}}
  \toprule
  Classnames word2vec & & \multicolumn{6}{c}{\textbf{Performance on class categories in mp500 (\%) }}\\
  \cmidrule(l){3-8}
  {\color{red} Different \# test classes} & & \multicolumn{2}{c}{\textbf{animals} (84)} &
  \multicolumn{2}{c}{\textbf{plants} (40)} &
  \multicolumn{2}{c}{\textbf{remain.} (376)}\\
  \cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8}
  \textbf{Classes excluded} & \textbf{\# excluded} & top-1
  & top-5     & top-1     & top-5      & top-1
  & top-5 \\
  \midrule
  None              & 0     & 24.30 & 53.50     &  4.47 & 16.21     & 15.24 & 37.71     \\
  All animal        & 398   &  1.88 &  9.24     &  5.99 & 17.31     & 15.39 & 37.35     \\
  Random non-animal & 398   & 23.64 & 51.79     &  4.07 & 12.81     & 10.64 & 29.69     \\
  All plant         & 31    & 23.69 & 53.93     &  3.40 & 14.21     & 15.33 & 37.74     \\
  Random non-plant  & 31    & 24.34 & 52.47     &  4.12 & 14.86     & 14.88 & 37.46     \\
\bottomrule
\end{tabular}

\end{table*}

